MirrorVLC: Optimal Mirror Placement for Multi-Element VLC Networks

Visible Light Communication (VLC) is a rapidly growing technology which can supplement the current radio frequency (RF) based wireless communication systems. VLC can play a huge part in solving the ever-increasing problem of spectrum scarcity because of the growing availability of Light Emitting Diodes (LEDs). One of the biggest advantages of VLC over other communication systems is that it can provide illumination and data communication simultaneously without needing any extra deployment. Although it is essential to provide data rate at a blazing speed to all the users nowadays, maintaining a satisfactory level in the distribution of lighting is also important. In this paper, we present a novel approach of using mirrors to enhance the illumination uniformity and throughput of an indoor multi-element VLC system architecture. In this approach, we improve the Signal-to-Interference plus Noise Ratio (SINR) of the system and overall illumination uniformity of the room by redirecting the reflected LED beams on the walls to darker spots with the use of mirrors. We formulate a joint optimization problem focusing on maximization of the SINR while maintaining a reasonable illumination uniformity across the room. We propose a two-stage solution of the optimization problem with optimization of illumination in the first stage and SINR at the second stage. We propose three different heuristic solutions for the second stage and analyze the performance of them, which demonstrates the advantages of each heuristic for different possible scenarios. We also show that about threefold increase in average illumination and fourfold increase in average throughput can be achieved when the mirror placement is applied which is a significant performance improvement.

==> code/diary <==
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.04s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.01 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.48 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.38 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Undefined function or variable 'writematrix'.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
writematrix(xi,fileID,'Delimiter','tab');
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.44 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Argument must contain a string.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save(fileID, 'xi', '-double', '-tab')
} 
matlab.internal.language.introspective.errorDocCallback('save')
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.03s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Unknown command option.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save(filename, 'xi', '-double', '-tab')
} 
matlab.internal.language.introspective.errorDocCallback('save')
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Unknown command option.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save('out.txt', 'xi', '-double', '-tab')
} 
matlab.internal.language.introspective.errorDocCallback('save')
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.60 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Unknown command option.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save('out.txt', 'xi', '-tab')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
[Warning: Saving sparse arrays to an ASCII file is unsupported.
	Variable 'chi_mz' not written to file.] 
[> In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 190)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',190,0)">line 190</a>)] 
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.38 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Unknown command option.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save('xi_values.txt', 'xi', '-ascii', '-int', '-tabs')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.32 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
[Warning: Saving sparse arrays to an ASCII file is unsupported.
	Variable 'chi_mz' not written to file.] 
[> In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 190)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',190,0)">line 190</a>)] 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
'%0.4g' is not a valid variable name.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 191)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',191,0)">line 191</a>)
save('P_m.txt', 'P_m','-ascii', '%0.4g', '-tabs')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.34 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('save')" style="font-weight:bold">save</a>
Unknown command option.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
save('xi_values.txt', 'xi', '-ascii', '-int64', '-tabs')
} 
matlab.internal.language.introspective.errorDocCallback('save')
matlab.internal.language.introspective.errorDocCallback('save')
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.41 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('fprintf')" style="font-weight:bold">fprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 190)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',190,0)">line 190</a>)
fprintf(fileID,'%d %d\n',chi_mz);
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.36 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('fprintf')" style="font-weight:bold">fprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 190)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',190,0)">line 190</a>)
fprintf(fileID,'%d \t',chi_mz);
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.28 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 87)" style="font-weight:bold">dlmwrite</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m',87,0)">line 87</a>)
FILENAME must be a string.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
dlmwrite(fileID, xi,' ')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.00s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.37 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Undefined function or variable 'finename'.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 189)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',189,0)">line 189</a>)
dlmwrite(finename, xi,' ')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('sprintf')" style="font-weight:bold">sprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)" style="font-weight:bold">dlmwrite</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m',169,0)">line 169</a>)
        str = sprintf(format,m(i,:));

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 191)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',191,0)">line 191</a>)
dlmwrite(filename, chi_mz,' ')
} 
mirrorvlc_main
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-04, 5e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.02s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 13 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (13 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [1e-04, 8e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 14 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (14 simplex iterations) in 0.36 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
 
Calling Gurobi 7.52: 893 variables, 658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 658 rows, 893 columns and 2287 nonzeros
Variable types: 889 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [1e-04, 8e-02]
Presolve removed 622 rows and 871 columns
Presolve time: 0.01s
Presolved: 36 rows, 22 columns, 146 nonzeros
Variable types: 18 continuous, 4 integer (4 binary)

Root relaxation: objective -5.224731e-03, 14 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0052247   -0.00522  0.00%     -    0s

Explored 0 nodes (14 simplex iterations) in 0.34 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.00522473 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.224730653940e-03, best bound -5.224730653940e-03, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.00522473
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('sprintf')" style="font-weight:bold">sprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)" style="font-weight:bold">dlmwrite</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m',169,0)">line 169</a>)
        str = sprintf(format,m(i,:));

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 191)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',191,0)">line 191</a>)
dlmwrite('chi_mz.txt', chi_mz,' ', m, Z)
} 
matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)
matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)
matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)
matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)
matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)
mirrorvlc_main
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [5e-06, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [4e-04, 8e-02]
Presolve removed 1588 rows and 2214 columns
Presolve time: 0.01s
Presolved: 70 rows, 39 columns, 262 nonzeros
Variable types: 35 continuous, 4 integer (4 binary)

Root relaxation: objective -1.385007e-02, 15 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0138501   -0.01385  0.00%     -    0s

Explored 0 nodes (15 simplex iterations) in 0.29 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0138501 

Optimal solution found (tolerance 1.00e-04)
Best objective -1.385006504194e-02, best bound -1.385006504194e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0138501
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('sprintf')" style="font-weight:bold">sprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)" style="font-weight:bold">dlmwrite</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m',169,0)">line 169</a>)
        str = sprintf(format,m(i,:));

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 191)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',191,0)">line 191</a>)
dlmwrite('chi_mz.txt', chi_mz, 'delimiter', ' ')
} 
P_m

P_m =

  Columns 1 through 12

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 13 through 24

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 25 through 36

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 37 through 48

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 49 through 60

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 61 through 65

    0.1000    0.1000    0.1000    0.1000    0.1000

I

I =

  Columns 1 through 12

    0.0143    0.0211    0.0211    0.0139    0.0219    0.0385    0.0383    0.0215    0.0219    0.0385    0.0383    0.0215

  Columns 13 through 16

    0.0143    0.0211    0.0211    0.0139

min(I)/mean(I)

ans =

    0.5815

mirrorvlc_main
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 8e-02]
Presolve removed 1575 rows and 2160 columns
Presolve time: 0.01s
Presolved: 83 rows, 93 columns, 1230 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -1.145793e-02, 39 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0114579   -0.01146  0.00%     -    0s

Explored 0 nodes (39 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0114579 

Optimal solution found (tolerance 1.00e-04)
Best objective -1.145793321911e-02, best bound -1.145793321911e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0114579
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('sprintf')" style="font-weight:bold">sprintf</a>
Function is not defined for sparse inputs.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('dlmwrite', '/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m', 169)" style="font-weight:bold">dlmwrite</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/toolbox/matlab/iofun/dlmwrite.m',169,0)">line 169</a>)
        str = sprintf(format,m(i,:));

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 191)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',191,0)">line 191</a>)
dlmwrite('chi_mz.txt', chi_mz, 'delimiter', ' ')
} 
P_m

P_m =

  Columns 1 through 12

    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200    0.0200

  Columns 13 through 24

    0.0855    0.1000    0.1000    0.0553    0.0200    0.1000    0.1000    0.0200    0.1000    0.1000    0.0200    0.0553

  Columns 25 through 36

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 37 through 48

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 49 through 60

    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000    0.1000

  Columns 61 through 65

    0.1000    0.1000    0.1000    0.1000    0.1000

I

I =

  Columns 1 through 12

    0.0115    0.0151    0.0153    0.0115    0.0160    0.0222    0.0229    0.0165    0.0160    0.0222    0.0229    0.0165

  Columns 13 through 16

    0.0115    0.0151    0.0153    0.0115

mirrorvlc_main
 
Calling Gurobi 7.52: 2254 variables, 1659 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1659 rows, 2254 columns and 6504 nonzeros
Variable types: 2246 continuous, 8 integer (8 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e+00]
Presolve removed 1575 rows and 2161 columns
Presolve time: 0.02s
Presolved: 84 rows, 93 columns, 1234 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -1.073768e-02, 72 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

     0     0   -0.01074    0    2          -   -0.01074      -     -    0s
H    0     0                      -0.0100013   -0.01074  7.36%     -    0s
H    0     0                      -0.0107116   -0.01074  0.24%     -    0s
     0     0   -0.01073    0    2   -0.01071   -0.01073  0.21%     -    0s

Cutting planes:
  MIR: 2

Explored 1 nodes (75 simplex iterations) in 0.53 seconds
Thread count was 4 (of 4 available processors)

Solution count 2: -0.0107116 -0.0100013 

Optimal solution found (tolerance 1.00e-04)
Best objective -1.071162506610e-02, best bound -1.071162506610e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0107116
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 8e-02]
Presolve removed 1575 rows and 2160 columns
Presolve time: 0.01s
Presolved: 83 rows, 93 columns, 1230 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -1.145793e-02, 39 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0114579   -0.01146  0.00%     -    0s

Explored 0 nodes (39 simplex iterations) in 0.45 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0114579 

Optimal solution found (tolerance 1.00e-04)
Best objective -1.145793321911e-02, best bound -1.145793321911e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0114579
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.02s
Presolved: 99 rows, 93 columns, 2282 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -3.541600e-02, 29 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0354160   -0.03542  0.00%     -    0s

Explored 0 nodes (29 simplex iterations) in 0.36 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.035416 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.541600118027e-02, best bound -3.541600118027e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.035416
 
 
Calling Gurobi 7.52: 2254 variables, 1659 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1659 rows, 2254 columns and 6583 nonzeros
Variable types: 2250 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 1e+02]
Presolve removed 0 rows and 1663 columns
Presolve time: 0.00s

Explored 0 nodes (0 simplex iterations) in 0.23 seconds
Thread count was 1 (of 4 available processors)

Solution count 0

Model is infeasible or unbounded
Best objective -, best bound -, gap -
------------------------------------------------------------
Status: Failed
Optimal value (cvx_optval): NaN
 
 
Calling Gurobi 7.52: 2254 variables, 1659 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1659 rows, 2254 columns and 6583 nonzeros
Variable types: 2250 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 1e+01]
Presolve removed 0 rows and 1663 columns
Presolve time: 0.00s

Explored 0 nodes (0 simplex iterations) in 0.24 seconds
Thread count was 1 (of 4 available processors)

Solution count 0

Model is infeasible or unbounded
Best objective -, best bound -, gap -
------------------------------------------------------------
Status: Failed
Optimal value (cvx_optval): NaN
 
 
Calling Gurobi 7.52: 2254 variables, 1659 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1659 rows, 2254 columns and 6583 nonzeros
Variable types: 2250 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 5e+00]
Presolve removed 0 rows and 1663 columns
Presolve time: 0.00s

Explored 0 nodes (0 simplex iterations) in 0.22 seconds
Thread count was 1 (of 4 available processors)

Solution count 0

Model is infeasible or unbounded
Best objective -, best bound -, gap -
------------------------------------------------------------
Status: Failed
Optimal value (cvx_optval): NaN
 
 
Calling Gurobi 7.52: 2254 variables, 1659 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1659 rows, 2254 columns and 6583 nonzeros
Variable types: 2250 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e+00]
Presolve removed 0 rows and 1663 columns
Presolve time: 0.00s

Explored 0 nodes (0 simplex iterations) in 0.13 seconds
Thread count was 1 (of 4 available processors)

Solution count 0

Model is infeasible or unbounded
Best objective -, best bound -, gap -
------------------------------------------------------------
Status: Failed
Optimal value (cvx_optval): NaN
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.02s
Presolved: 99 rows, 93 columns, 2282 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -3.541600e-02, 29 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0354160   -0.03542  0.00%     -    0s

Explored 0 nodes (29 simplex iterations) in 0.36 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.035416 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.541600118027e-02, best bound -3.541600118027e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.035416
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6495 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.03s
Presolved: 99 rows, 93 columns, 2282 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -3.541600e-02, 29 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0354160   -0.03542  0.00%     -    0s

Explored 0 nodes (29 simplex iterations) in 0.33 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.035416 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.541600118027e-02, best bound -3.541600118027e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.035416
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6499 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.01s
Presolved: 99 rows, 93 columns, 2286 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -3.566596e-02, 68 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0356660   -0.03567  0.00%     -    0s

Explored 0 nodes (68 simplex iterations) in 0.28 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.035666 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.566595642226e-02, best bound -3.566595642226e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.035666
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6602 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [4e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.01s
Presolved: 99 rows, 93 columns, 2389 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -7.268264e-02, 26 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0726826   -0.07268  0.00%     -    0s

Explored 0 nodes (26 simplex iterations) in 0.30 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0726826 

Optimal solution found (tolerance 1.00e-04)
Best objective -7.268264096115e-02, best bound -7.268264096115e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0726826
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6567 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.02s
Presolved: 99 rows, 93 columns, 2354 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -5.116508e-02, 34 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0511651   -0.05117  0.00%     -    0s

Explored 0 nodes (34 simplex iterations) in 0.29 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0511651 

Optimal solution found (tolerance 1.00e-04)
Best objective -5.116508495485e-02, best bound -5.116508495485e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0511651
 
 
Calling Gurobi 7.52: 13337 variables, 9808 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9808 rows, 13337 columns and 31287 nonzeros
Variable types: 13331 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 3e-01]
Presolve removed 9550 rows and 12918 columns
Presolve time: 0.06s
Presolved: 258 rows, 419 columns, 5790 nonzeros
Variable types: 413 continuous, 6 integer (6 binary)

Root relaxation: objective -3.922211e-01, 121 iterations, 0.01 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3922211   -0.39222  0.00%     -    0s

Explored 0 nodes (121 simplex iterations) in 0.50 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.392221 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.922211310116e-01, best bound -3.922211310116e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.392221
 
 
Calling Gurobi 7.52: 13337 variables, 9808 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9808 rows, 13337 columns and 31287 nonzeros
Variable types: 13331 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 8e-02]
Presolve removed 9550 rows and 12918 columns
Presolve time: 0.05s
Presolved: 258 rows, 419 columns, 5790 nonzeros
Variable types: 413 continuous, 6 integer (6 binary)

Root relaxation: objective -1.307404e-01, 112 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.1307404   -0.13074  0.00%     -    0s

Explored 0 nodes (112 simplex iterations) in 0.34 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.13074 

Optimal solution found (tolerance 1.00e-04)
Best objective -1.307403770039e-01, best bound -1.307403770039e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.13074
 
 
Calling Gurobi 7.52: 13338 variables, 9809 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9809 rows, 13338 columns and 31665 nonzeros
Variable types: 13332 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+01]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 4e+02]
Presolve removed 9551 rows and 12919 columns
Presolve time: 0.07s
Presolved: 258 rows, 419 columns, 5790 nonzeros
Variable types: 413 continuous, 6 integer (6 binary)

Root relaxation: objective -3.922211e-01, 119 iterations, 0.01 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3922211   -0.39222  0.00%     -    0s

Explored 0 nodes (119 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.392221 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.922211310116e-01, best bound -3.922211310116e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.392221
 
 
Calling Gurobi 7.52: 13338 variables, 9809 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9809 rows, 13338 columns and 31665 nonzeros
Variable types: 13332 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+01]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 5e+02]
Presolve removed 0 rows and 9811 columns
Presolve time: 0.03s

Explored 0 nodes (0 simplex iterations) in 0.17 seconds
Thread count was 1 (of 4 available processors)

Solution count 0

Model is infeasible or unbounded
Best objective -, best bound -, gap -
------------------------------------------------------------
Status: Failed
Optimal value (cvx_optval): NaN
 
 
Calling Gurobi 7.52: 13338 variables, 9809 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9809 rows, 13338 columns and 31665 nonzeros
Variable types: 13332 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+01]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 5e+02]
Presolve removed 9566 rows and 12919 columns
Presolve time: 0.06s
Presolved: 243 rows, 419 columns, 3670 nonzeros
Variable types: 413 continuous, 6 integer (6 binary)

Root relaxation: objective -3.922211e-01, 116 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3922211   -0.39222  0.00%     -    0s

Explored 0 nodes (116 simplex iterations) in 0.38 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.392221 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.922211310116e-01, best bound -3.922211310116e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.392221
 
 
Calling Gurobi 7.52: 13338 variables, 9809 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9809 rows, 13338 columns and 31665 nonzeros
Variable types: 13332 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+01]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 1e+02]
Presolve removed 9551 rows and 12919 columns
Presolve time: 0.07s
Presolved: 258 rows, 419 columns, 5790 nonzeros
Variable types: 413 continuous, 6 integer (6 binary)

Root relaxation: objective -3.907425e-01, 127 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3907425   -0.39074  0.00%     -    0s

Explored 0 nodes (127 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.390742 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.907424794664e-01, best bound -3.907424794664e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.390742
 
{Undefined function or variable 'cvx_begin'.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', 'C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m', 109)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m',109,0)">line 109</a>)
cvx_begin
} 
cd('C:\Users\si703115\Downloads\cvx-w64\cvx')
cvx_setup

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
Preferences: none found; defaults loaded.
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    No license installed.
No valid licenses found.
    <a href="http://cvxr.com/cvx/academic?c_act=fill&c_unm=si703115&c_hid=d89ef3109de1
">Click here</a> to fill out an academic license request
    for the username and first hostid listed above.
---------------------------------------------------------------------------
Setting CVX paths...done.
Saving updated path...done.
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
2 solvers initialized (* = default):
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
4 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
    Mosek      9.1.9      {cvx}\mosek\w64
        Using MOSEK with CVX requires an academic MOSEK license
        or a MOSEK-enabled CVX Professional license.
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------


Your MATLAB session has timed out.  All license keys have been returned.
uiopen('C:\Users\si703115\Downloads\cvx_license.dat',1)
cd('C:\Users\si703115\Downloads')
cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
File: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat
    Host ID: acbc32befd47, 82130fdf4c40
    Expiration: 2021-05-29 (320 days remaining)
    Status: INVALID:HOSTID,USER
     * None of the host IDs for this computer match those included in the license.
     *   License file:  acbc32befd47, 82130fdf4c40
     *   This computer: d89ef3109de1
     * The current username does not match those included in the license.
     *   License file: Sifat
     *   Current user: si703115
No valid licenses found.
    <a href="http://cvxr.com/cvx/academic?c_act=fill&c_unm=si703115&c_hid=d89ef3109de1
">Click here</a> to fill out an academic license request
    for the username and first hostid listed above.
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
2 solvers initialized (* = default):
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
4 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
    Mosek      9.1.9      {cvx}\mosek\w64
        Using MOSEK with CVX requires an academic MOSEK license
        or a MOSEK-enabled CVX Professional license.
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

web('http://cvxr.com/cvx/academic?c_act=fill&c_unm=si703115&c_hid=d89ef3109de1')
cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installing license:
    File: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_grbgetkey 7a70278c-a1ba-11ea-8930-0a7c4f30bdbe

---------------------------------------------------------------------------
CVX/Gurobi license key installer
---------------------------------------------------------------------------
Contacting the Gurobi Optimization license server...done.
The attempt to retrieve the license key failed with the following error:

    info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
error : ERROR 405: Cannot reinstall license 455126; get a new license from the Gurobi website

For information about this error, please consult the Gurobi documentation

    <a href="matlab: web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node5','-browser');">http://www.gurobi.com/documentation/5.5/quick-start-guide/node5</a>

Once you have rectified the error, please try again.
---------------------------------------------------------------------------
info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
error : ERROR 405: Cannot reinstall license 455126; get a new license from the Gurobi website
---------------------------------------------------------------------------
Now that the license has been retrieved, please run CVX_SETUP to configure
CVX to use the Gurobi solver with the new license.
---------------------------------------------------------------------------

cvx_grbgetkey fbf3b5ac-c51a-11ea-a7af-020d093b5256

---------------------------------------------------------------------------
CVX/Gurobi license key installer
---------------------------------------------------------------------------
Contacting the Gurobi Optimization license server...done.
The attempt to retrieve the license key failed with the following error:

    info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
info  : Key for license ID 469909 was successfully retrieved
info  : License expires at the end of the day on 2020-09-11
info  : Saving license key...
info  : License 469909 written to file C:\Users\si703115\AppData\Local\Temp\tpff5addb9_1a0a_4d39_95a0_97b35e0c1616\gurobi.lic

For information about this error, please consult the Gurobi documentation

    <a href="matlab: web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node5','-browser');">http://www.gurobi.com/documentation/5.5/quick-start-guide/node5</a>

Once you have rectified the error, please try again.
---------------------------------------------------------------------------
[Warning: Escaped character '\U' is not valid. See 'doc sprintf' for supported special characters.] 
[> In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_grbgetkey', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_grbgetkey.m', 338)" style="font-weight:bold">cvx_grbgetkey</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_grbgetkey.m',338,0)">line 338</a>)] 
info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
info  : Key for license ID 469909 was successfully retrieved
info  : License expires at the end of the day on 2020-09-11
info  : Saving license key...
info  : License 469909 written to file C:---------------------------------------------------------------------------
Now that the license has been retrieved, please run CVX_SETUP to configure
CVX to use the Gurobi solver with the new license.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_grbgetkey fbf3b5ac-c51a-11ea-a7af-020d093b5256

---------------------------------------------------------------------------
CVX/Gurobi license key installer
---------------------------------------------------------------------------
Contacting the Gurobi Optimization license server...done.
The attempt to retrieve the license key failed with the following error:

    info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
info  : Key for license ID 469909 was successfully retrieved
info  : License expires at the end of the day on 2020-09-11
info  : Saving license key...
info  : License 469909 written to file C:\Users\si703115\AppData\Local\Temp\tp78622686_b79d_405c_9af0_2af288c8a1f6\gurobi.lic

For information about this error, please consult the Gurobi documentation

    <a href="matlab: web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node5','-browser');">http://www.gurobi.com/documentation/5.5/quick-start-guide/node5</a>

Once you have rectified the error, please try again.
---------------------------------------------------------------------------
[Warning: Escaped character '\U' is not valid. See 'doc sprintf' for supported special characters.] 
[> In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_grbgetkey', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_grbgetkey.m', 338)" style="font-weight:bold">cvx_grbgetkey</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_grbgetkey.m',338,0)">line 338</a>)] 
info  : grbgetkey version 9.0.0, build v9.0.0rc2
info  : Contacting Gurobi key server...
info  : Key for license ID 469909 was successfully retrieved
info  : License expires at the end of the day on 2020-09-11
info  : Saving license key...
info  : License 469909 written to file C:---------------------------------------------------------------------------
Now that the license has been retrieved, please run CVX_SETUP to configure
CVX to use the Gurobi solver with the new license.
---------------------------------------------------------------------------

web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node5','-browser');
cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
3 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

uiopen('C:\gurobi752\win64\matlab\gurobi_setup.m',1)
gurobi_setup
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('gurobi_setup', 'C:\gurobi752\win64\matlab\gurobi_setup.m', 89)" style="font-weight:bold">gurobi_setup</a> (<a href="matlab: opentoline('C:\gurobi752\win64\matlab\gurobi_setup.m',89,0)">line 89</a>)
Invalid MEX-file 'C:\gurobi752\win64\matlab\gurobi.mexw64': Missing dependent shared libraries:
'gurobi60.dll' required by 'C:\gurobi752\win64\matlab\gurobi.mexw64'
'MSVCR90.dll' required by 'C:\gurobi752\win64\matlab\gurobi.mexw64'.
} 
home
cd home
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cd')" style="font-weight:bold">cd</a>
Cannot CD to C:\gurobi752\win64\matlab\home (Name is nonexistent or not a directory).
} 
cd('C:\Users\si703115\Downloads')
cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
4 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
    Gurobi_3   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
4 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
    Gurobi_3   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)
getenv('PATH')

ans =

    'C:\gurobi752\win64\bin;C:\WINDOWS\system32;C:\WINDOWS;C:\WINDOWS\System32\Wbem;C:\WINDOWS\System32\WindowsPowerShell\v1.0\;C:\Program Files\MATLAB\R2018b\runtime\win64;C:\Program Files\MATLAB\R2018b\bin;C:\Program Files\MATLAB\R2017b\runtime\win64;C:\Program Files\MATLAB\R2017b\bin;C:\Program Files\MiKTeX 2.9\miktex\bin\x64\;C:\WINDOWS\System32\OpenSSH\;C:\Users\si703115\AppData\Local\Microsoft\WindowsApps;C:\Users\si703115\AppData\Roaming\MiKTeX\2.9\miktex\bin\x64\;'

cvx_setup cvx_license.dat

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.2, Build 1148 (62bfcca)                  Tue Jan 28 00:51:35 2020
---------------------------------------------------------------------------
Installation info:
    Path: C:\Users\si703115\Downloads\cvx-w64\cvx
    MATLAB version: 9.5 (R2018b)
    OS: Windows 10 amd64 version 10.0
    Java version: 1.8.0_152
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        C:\Users\si703115\Downloads\cvx-w64\cvx\sedumi\.travis.yml
    These omissions may prevent CVX from operating properly.
    WARNING: The following extra files/directories were found:
        C:\Users\si703115\Downloads\cvx-w64\cvx\gurobi\w64\gurobi.lic
    These files may alter the behavior of CVX in unsupported ways.
Preferences: 
    Path: C:\Users\si703115\AppData\Roaming\MathWorks\MATLAB\cvx_prefs.mat
License host:
    Username: si703115
    Host ID: d89ef3109de1 (eth3,10.173.220.179)
Installed license:
    Also in file: cvx_license.dat
    Also in file: C:\Users\si703115\Downloads\cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat, si703115
    Host ID: acbc32befd47, 82130fdf4c40, d89ef3109de1
    Expiration: 2021-05-29 (320 days remaining)
    Status: verified
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
[Warning: Escaped character '\g' is not valid. See 'doc sprintf' for supported special characters.] 
[> In cvx_gurobi
  In cvx_gurobi
  In <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_setup', 'C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m', 83)" style="font-weight:bold">cvx_setup</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\cvx_setup.m',83,0)">line 83</a>)] 
5 shims found.
3 solvers initialized (* = default):
    Mosek      9.1.9      {cvx}\mosek\w64
 *  SDPT3      4.0        {cvx}\sdpt3
    SeDuMi     1.3.4      {cvx}\sedumi
4 solvers skipped:
    GLPK                  
        Could not find a GLPK installation.
    Gurobi     unknown    {cvx}\gurobi\w64
        No valid Gurobi license was found.
    Gurobi_2   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
    Gurobi_3   unknown    C:\gurobi752\win64\matlab
        Invalid MEX-file 'C:
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

cvx_solver gurobi
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_solver', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_solver.m', 46)" style="font-weight:bold">cvx_solver</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_solver.m',46,0)">line 46</a>)
Unknown, unusable, or missing solver: gurobi
} 
cvx_solver Gurobi
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_solver', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_solver.m', 46)" style="font-weight:bold">cvx_solver</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_solver.m',46,0)">line 46</a>)
Unknown, unusable, or missing solver: Gurobi
} 
 
Calling SDPT3 4.0: 2254 variables, 1659 equality constraints
------------------------------------------------------------
------------------------------------------------------------
Status: Error
Optimal value (cvx_optval): NaN
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_sdpt3>solve', 'C:\Users\si703115\Downloads\cvx-w64\cvx\shims\cvx_sdpt3.m', 131)" style="font-weight:bold">cvx_sdpt3>solve</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\shims\cvx_sdpt3.m',131,0)">line 131</a>)
SDTP3 does not support integer variables.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvxprob/solve', 'C:\Users\si703115\Downloads\cvx-w64\cvx\lib\@cvxprob\solve.m', 435)" style="font-weight:bold">cvxprob/solve</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\lib\@cvxprob\solve.m',435,0)">line 435</a>)
            [ x, status, tprec, iters ] = shim.solve( At, b, c, cones, quiet, prec, solv.settings,
            eargs{:} );

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_end', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m', 88)" style="font-weight:bold">cvx_end</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m',88,0)">line 88</a>)
        solve( prob );

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', 'C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m', 165)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m',165,0)">line 165</a>)
cvx_end
} 
cvx_solver Gurobi
cvx_save_prefs
Saving prefs...done.
mirrorvlc_main
 
Calling Gurobi 9.00: 2254 variables, 1659 equality constraints
------------------------------------------------------------
------------------------------------------------------------
Status: Error
Optimal value (cvx_optval): NaN
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_end', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m', 267)" style="font-weight:bold">cvx_end</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m',267,0)">line 267</a>)
model.quadcon must be a struct array with fields q, and rhs

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', 'C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m', 165)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m',165,0)">line 165</a>)
cvx_end
} 
opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m',267,0)
mirrorvlc_main
 
Calling Gurobi 9.00: 2253 variables, 1658 equality constraints
------------------------------------------------------------
------------------------------------------------------------
Status: Error
Optimal value (cvx_optval): NaN
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_end', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m', 267)" style="font-weight:bold">cvx_end</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m',267,0)">line 267</a>)
model.quadcon must be a struct array with fields q, and rhs

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', 'C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m', 165)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m',165,0)">line 165</a>)
cvx_end
} 
cvx_solver Mosek
mirrorvlc_main
 
Calling Mosek 9.1.9: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 9.1.9 (Build date: 2019-11-21 11:34:40)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: Windows/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 93 variables, 99 constraints, 2354 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        1        0        -5.1165084955e-02    -5.1165084955e-02    0.00e+00    0.0   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -5.116508495485e-02     
Best objective bound               : -5.116508495485e-02     
Construct solution objective       : Not employed
User objective cut value           : Not employed
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 9
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend optimizing the root     : 0.02
Mixed integer optimizer terminated. Time: 0.06

Optimizer terminated. Time: 0.09    


Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -5.1165084955e-02   nrm: 1e+00    Viol.  con: 5e-17    var: 7e-15    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 0.09    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.06    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0511651
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6531 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.01s
Presolved: 99 rows, 93 columns, 2318 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -4.368574e-02, 37 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0436857   -0.04369  0.00%     -    0s

Explored 0 nodes (37 simplex iterations) in 0.37 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0436857 

Optimal solution found (tolerance 1.00e-04)
Best objective -4.368573964081e-02, best bound -4.368573964081e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Gurobi 7.52: 13337 variables, 9808 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9808 rows, 13337 columns and 31289 nonzeros
Variable types: 13331 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 3e-01]
Presolve removed 9550 rows and 12912 columns
Presolve time: 0.05s
Presolved: 258 rows, 425 columns, 5798 nonzeros
Variable types: 419 continuous, 6 integer (6 binary)

Root relaxation: objective -3.565681e-01, 111 iterations, 0.01 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3565681   -0.35657  0.00%     -    0s

Explored 0 nodes (111 simplex iterations) in 0.33 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.356568 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.565680818868e-01, best bound -3.565680818868e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.356568
 
 
Calling Mosek 8.0.0.60: 13337 variables, 9808 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 9808            
  Cones                  : 0               
  Scalar variables       : 13337           
  Matrix variables       : 0               
  Integer variables      : 6               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.07
Presolved problem: 432 variables, 258 constraints, 5825 non-zeros
Presolved problem: 0 general integer, 6 binary, 426 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -3.5656808189e-01    NA          0.6   
0        1        0        0        -3.5656808189e-01    -3.5656808189e-01    0.00e+00    0.6   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -3.565680818868e-01     
Best objective bound               : -3.565680818868e-01     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 17
Number of simplex iterations       : 0
Time spend presolving the root     : 0.07
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.10
Mixed integer optimizer terminated. Time: 0.68

Optimizer terminated. Time: 1.25    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -3.5656808189e-01   nrm: 1e+00    Viol.  con: 7e-16    var: 8e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.25    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.68    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.356568
 
 
Calling Gurobi 7.52: 13337 variables, 9808 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 9808 rows, 13337 columns and 31289 nonzeros
Variable types: 13331 continuous, 6 integer (6 binary)
Coefficient statistics:
  Matrix range     [1e-04, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-02, 3e-01]
Presolve removed 9550 rows and 12912 columns
Presolve time: 0.08s
Presolved: 258 rows, 425 columns, 5798 nonzeros
Variable types: 419 continuous, 6 integer (6 binary)

Root relaxation: objective -3.565681e-01, 111 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.3565681   -0.35657  0.00%     -    0s

Explored 0 nodes (111 simplex iterations) in 0.51 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.356568 

Optimal solution found (tolerance 1.00e-04)
Best objective -3.565680818868e-01, best bound -3.565680818868e-01, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.356568
 
 
Calling Gurobi 9.00: 13337 variables, 9808 equality constraints
------------------------------------------------------------
------------------------------------------------------------
Status: Error
Optimal value (cvx_optval): NaN
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_end', 'C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m', 267)" style="font-weight:bold">cvx_end</a> (<a href="matlab: opentoline('C:\Users\si703115\Downloads\cvx-w64\cvx\commands\cvx_end.m',267,0)">line 267</a>)
model.quadcon must be a struct array with fields q, and rhs

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', 'C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m', 165)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('C:\Users\si703115\Dropbox\Sifat\MirrorVLC\code\mirrorvlc_main.m',165,0)">line 165</a>)
cvx_end
} 
cvx_solver

   Name     Status             Version   Location
------------------------------------------------------------
   Gurobi   selected,default   9.00      {cvx}\gurobi\w64
   Mosek                       9.1.9     {cvx}\mosek\w64
   SDPT3                       4.0       {cvx}\sdpt3
   SeDuMi                      1.3.4     {cvx}\sedumi

cd('C:\gurobi811\win64\matlab')
Your MATLAB session has timed out.  All license keys have been returned.
gurobi_setup
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('gurobi_setup', 'C:\gurobi811\win64\matlab\gurobi_setup.m', 89)" style="font-weight:bold">gurobi_setup</a> (<a href="matlab: opentoline('C:\gurobi811\win64\matlab\gurobi_setup.m',89,0)">line 89</a>)
Invalid MEX-file 'C:\gurobi811\win64\matlab\gurobi.mexw64': Missing dependent shared libraries:
'gurobi81.dll' required by 'C:\gurobi811\win64\matlab\gurobi.mexw64'
'MSVCR90.dll' required by 'C:\gurobi811\win64\matlab\gurobi.mexw64'.
} 
 
Calling Mosek 8.0.0.60: 4089 variables, 3008 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 3008            
  Cones                  : 0               
  Scalar variables       : 4089            
  Matrix variables       : 0               
  Integer variables      : 6               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.15
Presolved problem: 195 variables, 237 constraints, 4680 non-zeros
Presolved problem: 0 general integer, 6 binary, 189 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -7.5987355027e-02    NA          0.9   
0        1        0        0        -7.5987355027e-02    -7.5987355027e-02    0.00e+00    0.9   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -7.598735502709e-02     
Best objective bound               : -7.598735502709e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 10
Number of simplex iterations       : 0
Time spend presolving the root     : 0.15
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.13
Mixed integer optimizer terminated. Time: 1.20

Optimizer terminated. Time: 2.08    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -7.5987355027e-02   nrm: 1e+00    Viol.  con: 6e-17    var: 1e-12    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 2.08    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 1.20    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0759874
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.03
Presolved problem: 93 variables, 99 constraints, 2318 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.3685739641e-02    NA          0.5   
0        1        0        0        -4.3685739641e-02    -4.3685739641e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.368573964081e-02     
Best objective bound               : -4.368573964081e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 11
Number of simplex iterations       : 0
Time spend presolving the root     : 0.03
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.62

Optimizer terminated. Time: 1.10    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.3685739641e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.10    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.62    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 85 variables, 81 constraints, 1799 non-zeros
Presolved problem: 0 general integer, 4 binary, 81 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.7993928517e-02    NA          0.5   
0        1        0        0        -4.7993928517e-02    -4.7993928517e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.799392851680e-02     
Best objective bound               : -4.799392851680e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 9
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.01
Mixed integer optimizer terminated. Time: 0.62

Optimizer terminated. Time: 1.15    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.7993928517e-02   nrm: 1e+00    Viol.  con: 4e-17    var: 3e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.15    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.62    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0479939
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.04
Presolved problem: 93 variables, 99 constraints, 2318 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.3685739641e-02    NA          0.5   
0        1        0        0        -4.3685739641e-02    -4.3685739641e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.368573964081e-02     
Best objective bound               : -4.368573964081e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 11
Number of simplex iterations       : 0
Time spend presolving the root     : 0.04
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.63

Optimizer terminated. Time: 1.08    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.3685739641e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.08    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.63    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Gurobi 7.52: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1658 rows, 2253 columns and 6531 nonzeros
Variable types: 2249 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1559 rows and 2160 columns
Presolve time: 0.01s
Presolved: 99 rows, 93 columns, 2318 nonzeros
Variable types: 89 continuous, 4 integer (4 binary)

Root relaxation: objective -4.368574e-02, 37 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0436857   -0.04369  0.00%     -    0s

Explored 0 nodes (37 simplex iterations) in 0.34 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0436857 

Optimal solution found (tolerance 1.00e-04)
Best objective -4.368573964081e-02, best bound -4.368573964081e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 93 variables, 99 constraints, 2318 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.3685739641e-02    NA          0.4   
0        1        0        0        -4.3685739641e-02    -4.3685739641e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.368573964081e-02     
Best objective bound               : -4.368573964081e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 11
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.60

Optimizer terminated. Time: 1.08    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.3685739641e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.08    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.60    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 93 variables, 99 constraints, 2318 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.3685739641e-02    NA          0.4   
0        1        0        0        -4.3685739641e-02    -4.3685739641e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.368573964081e-02     
Best objective bound               : -4.368573964081e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 11
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.58

Optimizer terminated. Time: 1.00    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.3685739641e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.00    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.58    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 93 variables, 99 constraints, 2318 non-zeros
Presolved problem: 0 general integer, 4 binary, 89 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -4.3685739641e-02    NA          0.5   
0        1        0        0        -4.3685739641e-02    -4.3685739641e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -4.368573964081e-02     
Best objective bound               : -4.368573964081e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 11
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.63

Optimizer terminated. Time: 1.06    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -4.3685739641e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.06    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.63    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0436857
 
 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 78 variables, 75 constraints, 1102 non-zeros
Presolved problem: 0 general integer, 4 binary, 74 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -5.4122290622e-02    NA          0.4   
0        1        0        0        -5.4122290622e-02    -5.4122290622e-02    0.00e+00    0.4   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -5.412229062249e-02     
Best objective bound               : -5.412229062249e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 9
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.01
Mixed integer optimizer terminated. Time: 0.54

Optimizer terminated. Time: 1.00    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -5.4122290622e-02   nrm: 1e+00    Viol.  con: 5e-17    var: 0e+00    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.00    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.54    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0541223
 

------------------------------------------------------------------------
       Segmentation violation detected at Sat Jul 18 07:09:41 2020
------------------------------------------------------------------------

Configuration:
  Crash Decoding      : Disabled
  Crash Mode          : continue (default)
  Current Graphics Driver: Unknown hardware 
  Current Visual      : Quartz
  Default Encoding    : ISO-8859-1
  Host Name           : Sifat-Macbook.local
  MATLAB Architecture : maci64
  MATLAB Root         : /Applications/MATLAB_R2016a.app
  MATLAB Version      : 9.0.0.341360 (R2016a)
  OpenGL              : hardware
  Operating System    : Darwin 19.5.0 Darwin Kernel Version 19.5.0: Tue May 26 20:41:44 PDT 2020; root:xnu-6153.121.2~2/RELEASE_X86_64 x86_64
  Processor ID        : x86 Family 6 Model 61 Stepping 4, GenuineIntel
  Virtual Machine     : Java 1.7.0_75-b13 with Oracle Corporation Java HotSpot(TM) 64-Bit Server VM mixed mode
  Window System       : Quartz

Fault Count: 1


Abnormal termination:
Segmentation violation

Register State (from fault):
  RAX = 00000001054eb800  RBX = 0000000000000003
  RCX = 00000001054eb800  RDX = 0000000000000003
  RSP = 00007fff6d4f0d8b  RBP = 00007000103a3dc0
  RSI = 00007fa3e2600000  RDI = 0000000105403080

   R8 = 0000700000000000   R9 = 00007fff6d4ef385
  R10 = 0000000105402000  R11 = 00007fa3e2900000
  R12 = 00000000103a3dc0  R13 = 00007fa3e26cf410
  R14 = 000000010e14dab0  R15 = 00007fa3e26a9190

  RIP = 00007000103a3ed8  RFL = 00007fa3f47004a0

   CS = 00007fa3e26cedc0   FS = 00007000103a3e10   GS = 00007000103a3de0

Stack Trace (from fault):
[  0] 0x0000000107db8314 /Applications/MATLAB_R2016a.app/bin/maci64/libmwfl.dylib+00037652 _ZN2fl4diag15stacktrace_base7captureERKNS0_14thread_contextEm+00000052
[  1] 0x0000000107dbb899 /Applications/MATLAB_R2016a.app/bin/maci64/libmwfl.dylib+00051353 _ZN2fl4test17terminate_handledEv+00000937
[  2] 0x0000000107dbb26c /Applications/MATLAB_R2016a.app/bin/maci64/libmwfl.dylib+00049772 _ZN2fl4diag13terminate_logEPKcPK17__darwin_ucontext+00000188
[  3] 0x000000010aa749c0 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00428480 _Z32mnRunPathDependentInitializationv+00003024
[  4] 0x000000010aa74c92 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00429202 _Z32mnRunPathDependentInitializationv+00003746
[  5] 0x000000010aa72eea /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00421610 mnFatalSignalHandler+00000154
[  6] 0x00007fff6d52e5fd           /usr/lib/system/libsystem_platform.dylib+00013821 _sigtramp+00000029
[  7] 0x00000001054eb800                                   <unknown-module>+00000000
[  8] 0x000000010e14dac8 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07670472 _ZN5boost10shared_ptrIN9MathWorks3lxe7IndicesEEC2IS3_NS_6detail14sp_inplace_tagINS6_13sp_ms_deleterIS3_EEEEEEPT_T0_+00000280
[  9] 0x000000010e12c590 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07533968 _ZN5boost7variantINS_10shared_ptrIKN9MathWorks3lxe7IndicesEEENS3_6xvalueENS_6detail7variant5void_ESA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_SA_E27internal_apply_visitor_implINS9_9destroyerEPvEENT_11result_typeEiiRSF_T0_+00000080
[ 10] 0x000000010e14a56e /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07656814 _ZN9MathWorks3lxe9SubStructD2Ev+00000158
[ 11] 0x000000010e12ee4c /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07544396 _ZN9MathWorks3lxe22OverloadedObjectRplaceD0Ev+00000028
[ 12] 0x000000010b24bfd4 /Applications/MATLAB_R2016a.app/bin/maci64/libmwlxeutilities.dylib+00040916 _ZNK9MathWorks3utl10attachment6detachEv+00000020
[ 13] 0x000000010e122681 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07493249 _ZN9MathWorks3lxe28MxArrayOwningRplaceDecoratorD2Ev+00000033
[ 14] 0x000000010e1226ce /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07493326 _ZN9MathWorks3lxe28MxArrayOwningRplaceDecoratorD0Ev+00000014
[ 15] 0x000000010b24bfd4 /Applications/MATLAB_R2016a.app/bin/maci64/libmwlxeutilities.dylib+00040916 _ZNK9MathWorks3utl10attachment6detachEv+00000020
[ 16] 0x000000010e157419 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+07709721 _ZN9MathWorks3lxe9at_rparenEPvNS_2ts4TypeEPKvS1_S1_+00000841
[ 17] 0x000000010e1a9385 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+08045445 _ZN9MathWorks3lxe38cpp_primitive_template_fn_with_contextIXadL_ZNS0_9at_rparenEPvNS_2ts4TypeEPKvS2_S2_EEEEbS2_S4_S6_S2_S2_+00000021
[ 18] 0x000000010dd010b5 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+03162293 callPrimitiveWrapper+00000277
[ 19] 0x000000010dcec2b6 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+03076790 _ZN9MathWorks3lxe15ExecutionDriver9ThreadRunEv+00000630
[ 20] 0x000000010dcf05f0 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+03094000 _ZN9MathWorks3lxe12IrEngineImpl5ApplyERKN2ir6IrTreeEPvS6_+00000352
[ 21] 0x000000010df68c13 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05684243 _ZN9MathWorks3lxe17IrEngineDecorator5ApplyERKN2ir6IrTreeEPvS6_+00000211
[ 22] 0x000000010e07c2d6 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+06812374 _ZN9MathWorks3lxe27FileBasedMatlabCodeFunction14DispatchScriptEiPP11mxArray_tagiS4_+00000422
[ 23] 0x000000010ab7c4c9 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_dispatcher.dylib+00402633 _ZN8Mfh_file16dispatch_fh_implEMS_FviPP11mxArray_tagiS2_EiS2_iS2_+00000873
[ 24] 0x000000010ab7c8f3 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_dispatcher.dylib+00403699 _ZN8Mfh_file11dispatch_fhEiPP11mxArray_tagiS2_+00000035
[ 25] 0x000000010e085afe /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+06851326 _ZN9MathWorks3lxe17LxeDispatcherImpl12apply_handleEPNS0_29DispatcherFunctionHandleTokenEmPNS0_6xvalueEmPKS4_+00000910
[ 26] 0x000000010e1a8ac5 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+08043205 _ZN9MathWorks3lxe38cpp_primitive_template_fn_with_contextIXadL_ZNS0_16ans_apply_handleEPvNS_2ts4TypeEPKvS2_S2_EEEEbS2_S4_S6_S2_S2_+00000021
[ 27] 0x000000010dc0f177 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02171255 _ZN9MathWorks3lxe13IrInterpreter17ApplyCppPrimitiveEPN2ir4termES4_RKNS_2ts4TypeES8_+00000407
[ 28] 0x000000010dc0e36f /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02167663 _ZN9MathWorks3lxe13IrInterpreter31process_application_of_constantEPN2ir4termE+00001999
[ 29] 0x000000010dc0c838 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02160696 _ZN9MathWorks3lxe13IrInterpreter13applyConstantEPN2ir4termE+00000248
[ 30] 0x000000010dc0ad12 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02153746 _ZN9MathWorks3lxe12IRTreeWalker9applyTermEPN2ir4termE+00000098
[ 31] 0x000000010dc0b1df /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02154975 _ZN9MathWorks3lxe12IRTreeWalker11getNextIRPCENS0_9irpc_typeE+00000559
[ 32] 0x000000010dc0c529 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02159913 _ZN9MathWorks3lxe13IrInterpreter9tree_walkERKNS0_9irpc_typeES4_+00000185
[ 33] 0x000000010dc0c3f6 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+02159606 _ZN9MathWorks3lxe13IrInterpreter9InterpretEv+00000086
[ 34] 0x000000010dcecd13 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+03079443 _ZN9MathWorks3lxe15ExecutionDriver9ThreadRunEv+00003283
[ 35] 0x000000010dcf05f0 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+03094000 _ZN9MathWorks3lxe12IrEngineImpl5ApplyERKN2ir6IrTreeEPvS6_+00000352
[ 36] 0x000000010df68c13 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05684243 _ZN9MathWorks3lxe17IrEngineDecorator5ApplyERKN2ir6IrTreeEPvS6_+00000211
[ 37] 0x000000010df296ef /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05424879 _ZN9MathWorks3lxe9Evaluator15ApplyStatementsERKN2ir6IrTreeERNS0_18IEvaluationContextE+00000447
[ 38] 0x000000010df2b617 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05432855 _ZN9MathWorks3lxe9Evaluator17EvalStatementImplEPKcRNS0_18IEvaluationContextE+00000167
[ 39] 0x000000010df2b6e8 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05433064 _ZN9MathWorks3lxe9Evaluator13EvalStatementERKNSt3__112basic_stringIDsNS2_11char_traitsIDsEENS2_9allocatorIDsEEEERNS0_18IEvaluationContextE+00000136
[ 40] 0x000000010dfb17dc /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05982172 _ZN9MathWorks3lxe9LxeBridge7EvalCmdERKNSt3__112basic_stringIDsNS2_11char_traitsIDsEENS2_9allocatorIDsEEEEb+00000396
[ 41] 0x000000010dfb1687 /Applications/MATLAB_R2016a.app/bin/maci64/libmwm_lxe.dylib+05981831 _ZN9MathWorks3lxe9LxeBridge7EvalCmdERKNSt3__112basic_stringIDsNS2_11char_traitsIDsEENS2_9allocatorIDsEEEEb+00000055
[ 42] 0x000000010aff0bad /Applications/MATLAB_R2016a.app/bin/maci64/libmwbridge.dylib+00068525 _Z28evalCommandWithLongjmpSafetyRKNSt3__112basic_stringIDsNS_11char_traitsIDsEENS_9allocatorIDsEEEE+00000093
[ 43] 0x000000010aff1305 /Applications/MATLAB_R2016a.app/bin/maci64/libmwbridge.dylib+00070405 _Z8mnParserv+00001173
[ 44] 0x000000010aa35391 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00168849 _ZN3mcr7runtime17InterpreterThread4Impl30mnParser_on_interpreter_threadEP11mcrInstance+00000033
[ 45] 0x000000010aa37ec1 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00179905 _ZN3mcr7runtime17InterpreterThread4Impl22TypedInvocationRequestIvE29doNotRethrowMxArrayExceptionsERKN5boost8functionIFvvEEE+00000033
[ 46] 0x000000010aa38e6e /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00183918 _ZN5boost6detail12shared_countC2INS0_17task_shared_stateINS_3_bi6bind_tIvPFvRKNS_8functionIFvvEEEENS4_5list1INS4_5valueIS8_EEEEEEvEEEEPT_+00000734
[ 47] 0x000000010aa3852b /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00181547 _ZN5boost6detail22task_base_shared_stateIvE3runEv+00000059
[ 48] 0x000000010aa38458 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00181336 _ZN5boost13packaged_taskIvEclEv+00000024
[ 49] 0x000000010aa35873 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00170099 _ZN3mcr7runtime17InterpreterThread4Impl26invocation_request_handlerEl+00000035
[ 50] 0x000000010a90f390 /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00410512 _ZN3iqm23registerIqmPpeConditionEv+00003232
[ 51] 0x000000010a8f912e /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00319790 _ZN5boost6detail8function21function_obj_invoker0INSt3__18functionIFNS_3anyEvEEES5_E6invokeERNS1_15function_bufferE+00000030
[ 52] 0x000000010a8f8692 /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00317074 _ZN3iqm18PackagedTaskPlugin7executeEP15inWorkSpace_tagRN5boost10shared_ptrIN14cmddistributor17IIPCompletedEventEEE+00000258
[ 53] 0x000000010aa4b10f /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00258319 _ZN5boost10shared_ptrIN14cmddistributor17IIPCompletedEventEEC2IS2_NS_6detail14sp_inplace_tagINS5_13sp_ms_deleterIS2_EEEEEEPT_T0_+00001471
[ 54] 0x000000010a8d698b /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00178571 _ZNK3iqm17DefaultPacketInfo7executeEP15inWorkSpace_tag+00000299
[ 55] 0x000000010a8b836a /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00054122 _ZN3iqm10DefaultIqm7dequeueEN6mlutil14cmddistributor13WhenToDequeue13WhenToDequeueEN5boost8optionalINSt3__18functionIFvRKNS5_10shared_ptrINS_22IntermediatePacketInfoEEEEEEEENS6_ImEE+00002170
[ 56] 0x000000010a8c0e0b /Applications/MATLAB_R2016a.app/bin/maci64/libmwiqm.dylib+00089611 _ZN3iqm10DefaultIqm26isIqmUserEventsModeEnabledEv+00005099
[ 57] 0x0000000105901277 /Applications/MATLAB_R2016a.app/bin/maci64/libmwservices.dylib+01282679 _Z40svWS_ProcessPendingEventsWithLimitedRateb+00018487
[ 58] 0x00000001058fc1ff /Applications/MATLAB_R2016a.app/bin/maci64/libmwservices.dylib+01262079 _Z25svWS_ProcessPendingEventsiib+00000863
[ 59] 0x00000001058fbefb /Applications/MATLAB_R2016a.app/bin/maci64/libmwservices.dylib+01261307 _Z25svWS_ProcessPendingEventsiib+00000091
[ 60] 0x000000010aa35b3f /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00170815 _ZN3mcr7runtime17InterpreterThread4Impl14process_eventsERKN5boost10shared_ptrIS2_EE+00000191
[ 61] 0x000000010aa36086 /Applications/MATLAB_R2016a.app/bin/maci64/libmwmcr.dylib+00172166 _ZN3mcr7runtime17InterpreterThread4Impl3runER 
Calling Mosek 8.0.0.60: 2253 variables, 1658 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1658            
  Cones                  : 0               
  Scalar variables       : 2253            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.02
Presolved problem: 78 variables, 75 constraints, 1102 non-zeros
Presolved problem: 0 general integer, 4 binary, 74 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -5.4122290622e-02    NA          0.5   
0        1        0        0        -5.4122290622e-02    -5.4122290622e-02    0.00e+00    0.5   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -5.412229062249e-02     
Best objective bound               : -5.412229062249e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 9
Number of simplex iterations       : 0
Time spend presolving the root     : 0.02
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.01
Mixed integer optimizer terminated. Time: 0.58

Optimizer terminated. Time: 1.03    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -5.4122290622e-02   nrm: 1e+00    Viol.  con: 5e-17    var: 0e+00    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.03    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.58    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0541223
 
 
Calling Gurobi 6.00: 2253 variables, 1658 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Optimize a model with 1658 rows, 2253 columns and 6042 nonzeros
Coefficient statistics:
  Matrix range    [6e-05, 1e+00]
  Objective range [1e+00, 1e+00]
  Bounds range    [1e+00, 1e+00]
  RHS range       [3e-03, 3e-01]
Presolve removed 1577 rows and 2168 columns
Presolve time: 0.01s
Presolved: 81 rows, 85 columns, 1799 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -4.799393e-02, 47 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0479939   -0.04799  0.00%     -    0s

Explored 0 nodes (47 simplex iterations) in 0.02 seconds
Thread count was 4 (of 8 available processors)

Optimal solution found (tolerance 1.00e-04)
Best objective -4.799392851680e-02, best bound -4.799392851680e-02, gap 0.0%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0479939
 
 
Calling Mosek 8.0.0.60: 2287 variables, 1690 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1690            
  Cones                  : 0               
  Scalar variables       : 2287            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.04
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  

Objective of best integer solution : Not available.
Best objective bound               : Not available.
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 0
Number of interior point iterations: 0
Number of simplex iterations       : 0
Time spend presolving the root     : 0.04
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.00
Mixed integer optimizer terminated. Time: 0.58

Optimizer terminated. Time: 1.26    

Integer solution solution summary
  Problem status  : PRIMAL_INFEASIBLE
  Solution status : UNKNOWN
  Primal.  obj: 0.0000000000e+00    nrm: 0e+00    Viol.  con: 4e+01    var: 0e+00    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.26    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 0         time: 0.58    

------------------------------------------------------------
Status: Infeasible
Optimal value (cvx_optval): -Inf
 
 
Calling Mosek 8.0.0.60: 2287 variables, 1690 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1690            
  Cones                  : 0               
  Scalar variables       : 2287            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.06
Presolved problem: 85 variables, 97 constraints, 2587 non-zeros
Presolved problem: 0 general integer, 4 binary, 81 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -3.6397919017e-02    NA          0.8   
0        1        0        0        -3.6397919017e-02    -3.6397919017e-02    0.00e+00    0.8   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -3.639791901708e-02     
Best objective bound               : -3.639791901708e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 10
Number of simplex iterations       : 0
Time spend presolving the root     : 0.06
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.10
Mixed integer optimizer terminated. Time: 0.96

Optimizer terminated. Time: 1.65    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -3.6397919017e-02   nrm: 1e+00    Viol.  con: 4e-17    var: 3e-17    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.65    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.96    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0363979
 
 
Calling Mosek 8.0.0.60: 2287 variables, 1690 equality constraints
------------------------------------------------------------

MOSEK Version 8.0.0.60 (Build date: 2017-3-1 13:08:15)
Copyright (c) MOSEK ApS, Denmark. WWW: mosek.com
Platform: MACOSX/64-X86

Problem
  Name                   :                 
  Objective sense        : min             
  Type                   : LO (linear optimization problem)
  Constraints            : 1690            
  Cones                  : 0               
  Scalar variables       : 2287            
  Matrix variables       : 0               
  Integer variables      : 4               

Optimizer started.
Mixed integer optimizer started.
Threads used: 4
Presolve started.
Presolve terminated. Time = 0.04
Presolved problem: 85 variables, 97 constraints, 2587 non-zeros
Presolved problem: 0 general integer, 4 binary, 81 continuous
Clique table size: 0
BRANCHES RELAXS   ACT_NDS  DEPTH    BEST_INT_OBJ         BEST_RELAX_OBJ       REL_GAP(%)  TIME  
0        1        0        0        NA                   -2.3937626095e-02    NA          0.4   
0        1        0        0        -2.3937626095e-02    -2.3937626095e-02    0.00e+00    0.4   
An optimal solution satisfying the relative gap tolerance of 1.00e-02(%) has been located.
The relative gap is 0.00e+00(%).
An optimal solution satisfying the absolute gap tolerance of 0.00e+00 has been located.
The absolute gap is 0.00e+00.

Objective of best integer solution : -2.393762609515e-02     
Best objective bound               : -2.393762609515e-02     
Construct solution objective       : Not employed
Construct solution # roundings     : 0
User objective cut value           : 0
Number of cuts generated           : 0
Number of branches                 : 0
Number of relaxations solved       : 1
Number of interior point iterations: 16
Number of simplex iterations       : 0
Time spend presolving the root     : 0.04
Time spend in the heuristic        : 0.00
Time spend in the sub optimizers   : 0.00
  Time spend optimizing the root   : 0.02
Mixed integer optimizer terminated. Time: 0.55

Optimizer terminated. Time: 1.01    

Integer solution solution summary
  Problem status  : PRIMAL_FEASIBLE
  Solution status : INTEGER_OPTIMAL
  Primal.  obj: -2.3937626095e-02   nrm: 1e+00    Viol.  con: 3e-17    var: 2e-15    itg: 0e+00  
Optimizer summary
  Optimizer                 -                        time: 1.01    
    Interior-point          - iterations : 0         time: 0.00    
      Basis identification  -                        time: 0.00    
        Primal              - iterations : 0         time: 0.00    
        Dual                - iterations : 0         time: 0.00    
        Clean primal        - iterations : 0         time: 0.00    
        Clean dual          - iterations : 0         time: 0.00    
    Simplex                 -                        time: 0.00    
      Primal simplex        - iterations : 0         time: 0.00    
      Dual simplex          - iterations : 0         time: 0.00    
    Mixed integer           - relaxations: 1         time: 0.55    

------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1690 rows, 2287 columns and 7682 nonzeros
Variable types: 2283 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [6e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1577 rows and 2202 columns
Presolve time: 0.03s
Presolved: 113 rows, 85 columns, 3375 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -2.393763e-02, 73 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0239376   -0.02394  0.00%     -    0s

Explored 0 nodes (73 simplex iterations) in 0.38 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0239376 

Optimal solution found (tolerance 1.00e-04)
Best objective -2.393762609515e-02, best bound -2.393762609515e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1690 rows, 2287 columns and 7350 nonzeros
Variable types: 2283 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1602 rows and 2214 columns
Presolve time: 0.03s
Presolved: 88 rows, 73 columns, 1896 nonzeros
Variable types: 69 continuous, 4 integer (4 binary)

Root relaxation: objective -2.076690e-02, 72 iterations, 0.01 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0207669   -0.02077  0.00%     -    0s

Explored 0 nodes (72 simplex iterations) in 0.51 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0207669 

Optimal solution found (tolerance 1.00e-04)
Best objective -2.076690267678e-02, best bound -2.076690267678e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0207669
 
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1690 rows, 2287 columns and 7350 nonzeros
Variable types: 2283 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [2e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [2e-03, 3e-01]
Presolve removed 1602 rows and 2214 columns
Presolve time: 0.03s
Presolved: 88 rows, 73 columns, 1896 nonzeros
Variable types: 69 continuous, 4 integer (4 binary)

Root relaxation: objective -2.076690e-02, 72 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0207669   -0.02077  0.00%     -    0s

Explored 0 nodes (72 simplex iterations) in 0.32 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0207669 

Optimal solution found (tolerance 1.00e-04)
Best objective -2.076690267678e-02, best bound -2.076690267678e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0207669
 
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
------------------------------------------------------------
Status: Error
Optimal value (cvx_optval): NaN
 
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx_end', '/Applications/MATLAB_R2016a.app/cvx/commands/cvx_end.m', 267)" style="font-weight:bold">cvx_end</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/cvx/commands/cvx_end.m',267,0)">line 267</a>)
Gurobi error 10009: License expired 2020-07-28 - license file '/Users/Sifat/.matlab/cvx_gurobi.lic'
Please consult the Gurobi Quick Start Guide for details on setting up a license.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('mirrorvlc_main', '/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m', 71)" style="font-weight:bold">mirrorvlc_main</a> (<a href="matlab: opentoline('/Users/Sifat/Dropbox/Sifat/MirrorVLC/code/mirrorvlc_main.m',71,0)">line 71</a>)
cvx_end
} 
grbgetkey fbf3b5ac-c51a-11ea-a7af-020d093b5256
{Undefined function or variable 'grbgetkey'.
} 
cvx where
{Error using <a href="matlab:matlab.internal.language.introspective.errorDocCallback('sparse')" style="font-weight:bold">sparse</a>
sparse(A) does not accept char inputs A.  Use sparse(double(A)) instead.

Error in <a href="matlab:matlab.internal.language.introspective.errorDocCallback('cvx', '/Applications/MATLAB_R2016a.app/cvx/lib/@cvx/cvx.m', 28)" style="font-weight:bold">cvx</a> (<a href="matlab: opentoline('/Applications/MATLAB_R2016a.app/cvx/lib/@cvx/cvx.m',28,0)">line 28</a>)
            v = class( struct( 'size_', size( s ), 'basis_', sparse( s(:).' ), 'dual_', '', 'dof_', [], 'slow_', nnz(
            isinf( s ) | isnan( s ) ) ~= 0 ), 'cvx', cvxobj );
} 
cvx
 
ans =
 
    cvx empty expression (0x0 matrix)
 
cvx_grbgetkey fbf3b5ac-c51a-11ea-a7af-020d093b5256

---------------------------------------------------------------------------
CVX/Gurobi license key installer
---------------------------------------------------------------------------
Contacting the Gurobi Optimization license server...done.
The attempt to retrieve the license key failed with the following error:

    ERROR 405: Cannot reinstall license 469909; get a new license from the Gurobi website
For information about this error, please consult the Gurobi documentation

    <a href="matlab: web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node5','-browser');">http://www.gurobi.com/documentation/5.5/quick-start-guide/node5</a>

Once you have rectified the error, please try again.
---------------------------------------------------------------------------
Gurobi license key client (version 7.5.2)
Copyright (c) 2017, Gurobi Optimization, Inc.

-------------------------------
Contacting Gurobi key server...
-------------------------------

ERROR 405: Cannot reinstall license 469909; get a new license from the Gurobi website

---------------------------------------------------------------------------
Now that the license has been retrieved, please run CVX_SETUP to configure
CVX to use the Gurobi solver with the new license.
---------------------------------------------------------------------------

cvx_grbgetkey 64a1615e-d195-11ea-a698-0a7c4f30bdbe

---------------------------------------------------------------------------
CVX/Gurobi license key installer
---------------------------------------------------------------------------
Contacting the Gurobi Optimization license server...done.
Download successful. The license can be found at

    /Users/Sifat/.matlab/cvx_gurobi.lic

The license will expire at the end of the day on 2020-09-27.
---------------------------------------------------------------------------
WARNING: This license is not a CVX-specific license. It will still work with
CVX; however, if you also wish to use it with other applications, then we
strongly recommend that you copy it to a standard Gurobi location. Consult
the following Gurobi documentation for more information:

    <a href="matlab: web('http://www.gurobi.com/documentation/5.5/quick-start-guide/node8','-browser');">http://www.gurobi.com/documentation/5.5/quick-start-guide/node8</a>

For instance, to move this file to the standard home directory location,
copy and paste this command into your MATLAB command line:

   movefile /Users/Sifat/.matlab/cvx_gurobi.lic ~/gurobi.lic
---------------------------------------------------------------------------
Now that the license has been retrieved, please run CVX_SETUP to configure
CVX to use the Gurobi solver with the new license.
---------------------------------------------------------------------------

cvx_setup

---------------------------------------------------------------------------
CVX: Software for Disciplined Convex Programming       (c)2014 CVX Research
Version 2.1, Build 1123 (cff5298)                  Sun Dec 17 18:58:10 2017
---------------------------------------------------------------------------
Installation info:
    Path: /Applications/MATLAB_R2016a.app/cvx
    MATLAB version: 9.0 (R2016a)
    OS: Mac OS X x86_64 version 10.15.6
    Java version: 1.7.0_75
Verfying CVX directory contents:
    WARNING: The following files/directories are missing:
        /Applications/MATLAB_R2016a.app/cvx/examples/ + 505 files, 30 subdirectories
    These omissions may prevent CVX from operating properly.
Preferences: 
    Path: /Users/Sifat/.matlab/cvx_prefs.mat
License host:
    Username: Sifat
    Host ID: acbc32befd47 (en0)
Installed license:
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat
    Host ID: acbc32befd47, 82130fdf4c40
    Expiration: 2021-05-29 (304 days remaining)
    Status: verified
Other license found:
    File: /Applications/MATLAB_R2016a.app/cvx/cvx_license.dat
    Organization: University of Central Florida
    Contact: Sifat Ibne Mushfique (sifat.im@knights.ucf.edu)
    License type: academic
    Named user: Sifat
    Host ID: acbc32befd47
    Expiration: 2019-11-13 (259 days ago)
    Status: invalid:expired
---------------------------------------------------------------------------
Setting CVX paths...already set!
Searching for solvers...5 shims found.
2 solvers initialized (* = default):
 *  Gurobi   7.52        {cvx}/gurobi/maci64
    Mosek    8.0.0.60    {cvx}/mosek/maci64
3 solvers skipped:
    GLPK                 
        Could not find a GLPK installation.
    SDPT3                
        Could not find a SDPT3 installation.
    SeDuMi               
        Could not find a SeDuMi installation.
Saving updated preferences...done.
Testing with a simple model...done!
---------------------------------------------------------------------------
To change the default solver, type "cvx_solver <solver_name>".
To save this change for future sessions, type "cvx_save_prefs".
Please consult the users' guide for more information.
---------------------------------------------------------------------------

mirrorvlc_main
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1690 rows, 2287 columns and 7682 nonzeros
Variable types: 2283 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [6e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1577 rows and 2202 columns
Presolve time: 0.02s
Presolved: 113 rows, 85 columns, 3375 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -2.393763e-02, 73 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0239376   -0.02394  0.00%     -    0s

Explored 0 nodes (73 simplex iterations) in 0.31 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0239376 

Optimal solution found (tolerance 1.00e-04)
Best objective -2.393762609515e-02, best bound -2.393762609515e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 
 
Calling Gurobi 7.52: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Academic license - for non-commercial use only
Optimize a model with 1690 rows, 2287 columns and 7682 nonzeros
Variable types: 2283 continuous, 4 integer (4 binary)
Coefficient statistics:
  Matrix range     [6e-05, 1e+00]
  Objective range  [1e+00, 1e+00]
  Bounds range     [1e+00, 1e+00]
  RHS range        [3e-03, 3e-01]
Presolve removed 1577 rows and 2202 columns
Presolve time: 0.03s
Presolved: 113 rows, 85 columns, 3375 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -2.393763e-02, 73 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0239376   -0.02394  0.00%     -    0s

Explored 0 nodes (73 simplex iterations) in 0.35 seconds
Thread count was 4 (of 4 available processors)

Solution count 1: -0.0239376 

Optimal solution found (tolerance 1.00e-04)
Best objective -2.393762609515e-02, best bound -2.393762609515e-02, gap 0.0000%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 
 
Calling Gurobi 6.00: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Optimize a model with 1690 rows, 2287 columns and 7682 nonzeros
Coefficient statistics:
  Matrix range    [6e-05, 1e+00]
  Objective range [1e+00, 1e+00]
  Bounds range    [1e+00, 1e+00]
  RHS range       [3e-03, 3e-01]
Presolve removed 1577 rows and 2202 columns
Presolve time: 0.01s
Presolved: 113 rows, 85 columns, 3375 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -2.393763e-02, 104 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0239376   -0.02394  0.00%     -    0s

Explored 0 nodes (104 simplex iterations) in 0.03 seconds
Thread count was 4 (of 8 available processors)

Optimal solution found (tolerance 1.00e-04)
Best objective -2.393762609515e-02, best bound -2.393762609515e-02, gap 0.0%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 
 
Calling Gurobi 6.00: 2287 variables, 1690 equality constraints
------------------------------------------------------------
Gurobi optimizer, licensed to CVX for CVX
Optimize a model with 1690 rows, 2287 columns and 7682 nonzeros
Coefficient statistics:
  Matrix range    [6e-05, 1e+00]
  Objective range [1e+00, 1e+00]
  Bounds range    [1e+00, 1e+00]
  RHS range       [3e-03, 3e-01]
Presolve removed 1577 rows and 2202 columns
Presolve time: 0.01s
Presolved: 113 rows, 85 columns, 3375 nonzeros
Variable types: 81 continuous, 4 integer (4 binary)

Root relaxation: objective -2.393763e-02, 104 iterations, 0.00 seconds

    Nodes    |    Current Node    |     Objective Bounds      |     Work
 Expl Unexpl |  Obj  Depth IntInf | Incumbent    BestBd   Gap | It/Node Time

*    0     0               0      -0.0239376   -0.02394  0.00%     -    0s

Explored 0 nodes (104 simplex iterations) in 0.02 seconds
Thread count was 4 (of 8 available processors)

Optimal solution found (tolerance 1.00e-04)
Best objective -2.393762609515e-02, best bound -2.393762609515e-02, gap 0.0%
------------------------------------------------------------
Status: Solved
Optimal value (cvx_optval): +0.0239376
 


==> makefile <==
DOCUMENT := TCCN_2019_Main
BINDIR := .
all:
	pdflatex $(DOCUMENT)
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT)
	pdflatex $(DOCUMENT)
#	mv $(DOCUMENT).dvi $(BINDIR)
#	dvips $(BINDIR)/$(DOCUMENT).dvi $(DVI_OPTIONS) -o $(BINDIR)/$(DOCUMENT).ps 
	\rm -rf *.aux *.dvi  *.log *.bbl *.blg *.toc *.lof
#	ps2pdf $(PS2PDF_OPTIONS) $(BINDIR)/$(DOCUMENT).ps $(BINDIR)/$(DOCUMENT).pdf
	@echo -e "\nCompiled with version:" $(CURRENT_COMP) "\n"
	open $(BINDIR)/$(DOCUMENT).pdf &
#	#evince $(BINDIR)/$(DOCUMENT).pdf &

.PHONY: clean
clean:
	@\rm -rf *.gz *.r* *.aux *.dvi *.log *.ps *.pdf *.bbl *.blg *.toc *.lof *.idx $(BINDIR)/*.dvi $(BINDIR)/*.ps  $(BINDIR)/*.pdf
	@echo "Cleaning directories"


